Input Selection for Bandwidth-Limited Neural Network Inference

Data are often accommodated on centralized storage servers. This is the case, for instance, in remote sensing and astronomy, where projects produce several petabytes of data every year. While machine learning models are often trained on relatively small subsets of the data, the inference phase typically requires transferring significant amounts of data between the servers and the clients. In many cases, the bandwidth available per user is limited, which then renders the data transfer to be one of the major bottlenecks. In this work, we propose a framework that automatically selects the relevant parts of the input data for a given neural network. The model as well as the associated selection masks are trained simultaneously such that a good model performance is achieved while only a minimal amount of data is selected. During the inference phase, only those parts of the data have to be transferred between the server and the client. We propose both instance-independent and instance-dependent selection masks. The former ones are the same for all instances to be transferred, whereas the latter ones allow for variable transfer sizes per instance. Our experiments show that it is often possible to significantly reduce the amount of data needed to be transferred without affecting the model quality much.

==> prev_reviews.tex <==



Previous versions of this manuscript were submitted to NeurIPS 2019, ICLR 2020, and KDD 2020. In general, the reviews were positive. The reviewers main concerns were a lack of comparison with other baselines as well as a (potential) lack of novelty.

The meta-review for this year's KDD conference was the following:

---- META-REVIEW KDD 2020 ----
While the reviewers found a lot to like, they all agreed that the paper had some weaknesses
1)      The paper lacks comparison with other current deep learning methods. There is no baseline in the experiments.
2)      The ranges of the parameter λ vary greatly in Fig 9, Fig 12, Fig 14 and Fig 17. The paper should to explain more why they are so different among different datasets.
3)      The paper needs to explain its novelty more clearly. One reviewer noted “ It borrows ideas from active learning to describe how masks can be used to reduce the communication cost of remote sensing”. 
-----------------------------

The last point was raised by one of the three reviewers, who pointed out that our work would be an active learning approach and connected to federated learning. We regret this misunderstanding and would like to stress that this is, in our opinion, clearly not the case (instead, we consider our approach as a specialized feature selection scheme).

We have carefully revised our manuscript and significantly extended our approach, our experiments, and our manuscript. In particular, the following changes and additions have been made:

(1) We have rewritten the motivation and are now emphasizing the applicability of our approach for real-world settings in more detail. We also highlight the novel contributions made.
(2) We extended our work to dynamic scenarios as requested by reviewer #3 of NeurIPS 2019.
(3) We have streamlined and simplified our approach.
(4) Almost all experiments have been recomputed from scratch (e.g. without Gumbel noise). We have also added additional parameter analyses and further experiments (e.g., dynamic ship classification)
(5) We have added comprehensive supplemental material, which includes, among other things, a detailed description of the experimental setting, details for reproducing our results, and various experiments beyond the ones provided in the manuscript.

We would like to point out that the initial version of our manuscript, which did not contain any dynamic masks, was evaluated quite positively at NeurIPS 2019 (just below the acceptance threshold). More precisely, we got the scores 6,7, and 4 for our submission "Learning Selection Masks for Deep Neural Networks" (paper id: 7524). The NeurIPS 2019 version of the manuscript can be found on arxiv (https://arxiv.org/abs/1906.04673v1). For the sake of completeness, we have also attached the NeurIPS 2019 post-rebuttal reviews below.

We have incorporated all the issues raised by the reviewers and sincerely hope that the considerably updated version of our manuscript will now satisfy the reviewers.


--- Post-Rebuttal Responses NeurIPS2019 ---

Reviewer #1
I carefully read the rebuttal and also comments of the other two reviewers. The rebuttal has addressed most of my concerns. I would like to upgrade the rating to "6".
3. Please provide an "overall score" for this submission.
6: Marginally above the acceptance threshold. I tend to vote for accepting this submission, but rejecting it would not be that bad.
4. Please provide a "confidence score" for your assessment of this submission.
5: You are absolutely certain about your assessment. You are very familiar with the related work.
5. Improvements: What would the authors have to do for you to increase your score?
See detailed comments.

Reviewer #2
I was satisfied with the rebuttal, which addressed my concerns and provides additional value to the paper. I'll vote (but won't argue) for acceptance -- so my score goes up one notch.
3. Please provide an "overall score" for this submission.
7: A good submission; an accept. I vote for accepting this submission, although I would not be upset if it were rejected.
4. Please provide a "confidence score" for your assessment of this submission.
4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
5. Improvements: What would the authors have to do for you to increase your score?
Improvements were fairly minor and noted above.

Reviewer #3
Thank you to the authors for their rebuttal. In the rebuttal, the authors have clarified the practical scenario that the work is targeting, which is 'client-side' masking of data requests, where no 'server-side' computation of reduced features is possible.

In my view, there are two major limitations to the paper:
1) This scenario, in practice, is a major restriction, and can almost always surmounted. Based on the manuscript and the rebuttal I remain unconvinced that this is a common scenario (features can almost always be trained, precomputed, etc. ahead of time, which would make this approach uncompetitive, as discussed in my original review above)
2) Assuming that this scenario is the reality, the investigation falls severely short of a NeurIPS quality submission:
- The approach is completely ad hoc. In particular, it is not clear what the benefit pre-defining arbitrary classes of masks is. It seems like a major limitation, and the problem is not approached in a rigorous manner.
- The approach is not compared to previous work, and put properly in context with the SOTA. Feature selection is a heavily studied problem, and is not clear that their approach would have any advantage over simple lasso, group lasso, or generalized relaxed feature selection approaches. Yes, GS is the latest way of doing this, but that does not absolve the authors from comparing to other approaches.
- From a practical standpoint, any client-side defined masking should be interactive and iterative, and as such highly context dependent. I remain unconvinced that this is application-specific SOTA work as claimed.

In summary, the submission falls far below the bar for acceptance at NeurIPS for reasons cited above.
3. Please provide an "overall score" for this submission.
4: An okay submission, but not good enough; a reject. I vote for rejecting this submission, although I would not be upset if it were accepted.
4. Please provide a "confidence score" for your assessment of this submission.
3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.
5. Improvements: What would the authors have to do for you to increase your score?
Stronger baselines and defense of approach.
-------------------------------------------

